Self-Organized Polynomial-Time Coordination Graphs

Coordination graph is a promising approach to model agent collaboration in multi-agent reinforcement learning. It conducts a graph-based value factorization and induces explicit coordination among agents to complete complicated tasks. However, one critical challenge in this paradigm is the complexity of greedy action selection with respect to the factorized values. It refers to the decentralized constraint optimization problem (DCOP), which and whose constant-ratio approximation are NP-hard problems. To bypass this systematic hardness, this paper proposes a novel method, named Self-Organized Polynomial-time Coordination Graphs (SOP-CG), which uses structured graph classes to guarantee the accuracy and the computational efficiency of collaborated action selection. SOP-CG employs dynamic graph topology to ensure sufficient value function expressiveness. The graph selection is unified into an end-to-end learning paradigm. In experiments, we show that our approach learns succinct and well-adapted graph topologies, induces effective coordination, and improves performance across a variety of cooperative multi-agent tasks.

==> 5_experiments_v0.tex <==
\section{Experiments}
In this section, we conduct experiments to answer the following questions: (1) Does the class of polynomial-time coordination graphs improve our performance (see Section~\ref{didactic_example})? (2) How well does SOP-CG perform on complex cooperative multi-agent tasks (see Fig.~\ref{figure:performance})? (3) Can SOP-CG extract interpretable dynamic coordination structures (see Fig.~\ref{figure:chase_illustration})?  %For evaluation, all learning curves are smoothed over 5 random seeds.

\subsection{Didactic example}
\label{didactic_example}

\begin{figure}[t]
    \centering
    \vspace{-3mm}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sensor_a.pdf}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sensor_b.pdf}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/sensor_c.pdf}
    \end{minipage}
    \caption{Ablation studies on Sensor-network: (a) comparison against DCG with online data collection; (b) comparison against DCG with offline dataset; (c) comparison with static topologies.}
    \label{figure:sensor_curves}
\end{figure}

% \begin{figure}[t]
%     \begin{minipage}{0.3\textwidth}
%         \centering
%         \includegraphics[height=3.1cm]{figures/sensor-snapshot.png}
%     \end{minipage}
%     \begin{minipage}{0.69\textwidth}
%         \centering
%         \scriptsize
%         \begin{tabular}{|c|c|c|c|}\hline
%         DCG  & $q_7$ & $q_8$  & $q_{78}$ \\ \hline
%         \multirow{2}{*}{Largest action (pair) values} & $-0.248$ & $-0.239$ & $-0.003$ \\ \cline{2-4} 
%          & $\bm{-0.484}$ & $-0.519$  & $-0.004$ \\ \hline
%          Value of best action (pair) & $\bm{-0.484}$ & $\bm{-0.607}$ & $\bm{-0.031}$ \\ \hline \hline
%          SOP-CG (tree)  & $q_7$ & $q_8$  & $q_{78}$ \\ \hline
%         \multirow{2}{*}{Largest action (pair) values} & $-0.011$ & $-0.163$ & $\bm{2.323}$ \\ \cline{2-4} 
%          & $-0.835$ & $\bm{-0.731}$  & $-0.101$ \\ \hline
%          Value of best action (pair) & $\bm{-0.900}$ & $\bm{-0.731}$ & $\bm{2.323}$ \\ \hline
%         \end{tabular}
%     \end{minipage}
%     \caption{Case study on Sensor-Network. Left: A snapshot of Sensor-Network; Right: Corresponding values learned by SOP-CG (tree) and DCG. The table shows the largest two action (pair) values as well as value of the best action (pair) of the utilities and payoff. In our algorithm, the individual utilities $q_7, q_8$ suggest agent 7 and 8 to keep no operation (with values $-0.011$ and $-0.163$ respectively). The pairwise payoff $q_{78}$ learns a large value ($2.323$) for coordinated actions so that the agents are forced to scan the target. By contrast, the payoff function $q_{78}$ learned by DCG fails to differentiate the effect of different action pairs, so both agents stay no operation.}
%     \label{sensor}
% \end{figure}




\begin{wrapfigure}[9]{r}{0.3\linewidth}
    \centering
    \vspace{-4mm}
    \includegraphics[width=\linewidth]{figures/sensor-illustration.png}
    \vspace{-7mm}
    \caption{Sensor-network.}
    \label{figure:sensor_illustration}
\end{wrapfigure}

We first study a didactic example to demonstrate two main contributions of this paper: (a) harnessing polynomial-time coordination graphs to obtain optimality guarantee of the induced DCOPs; (b) maintaining function expressiveness by incorporating a class of structured graphs into the Q-learning framework. We conduct ablation studies on \emph{Sensor-network}, which is a classic task for testing multi-agent coordination \citep{lesser2003distributed,zhang2011coordinated}. We adopt the same task configuration as \cite{wang2021context}. As illustrated in Fig.~\ref{figure:sensor_illustration}, 15 sensor agents are arranged as a $3\times 5$ matrix while three targets randomly walk in the same grid space. At each timestep, an agent can choose to scan one of the eight nearby positions (inducing a cost) or perform no operation. If two or more agents scan the target simultaneously, the target is captured and produces a positive joint reward. We compare our algorithm with DCG \citep{bohmer2020deep} on this game. The default implementation of DCG uses a fully connected coordination graph. In addition, DCG provides alternative implementations on two static graphs \emph{Line} (agent $i$ is connected with agent $i-1$ and $i+1$) and \emph{Star} (agent $1$ is linked with others), which are two special instances of $\mathcal{G}_T$. SOP-CG ($\mathcal{G}_T$) has absolutely higher function expressiveness than DCG (line) and DCG (star).

For the first contribution, we verify that the optimality guarantee of the induced DCOP in our algorithm improve the performance. We test these algorithms in both online (Fig.~\ref{figure:sensor_curves}a) and offline learning (Fig.~\ref{figure:sensor_curves}b) settings. For fair evaluation, we train DCG (line) and collect 15K experienced episodes throughout the training process to set up the diverse offline dataset. As shown in Fig.~\ref{figure:sensor_curves}(a-b), SOP-CG outperforms DCG in both settings. In the offline setting, as the dataset is fixed for both algorithms, the main difference between SOP-CG and DCG lies in the construction of one-step TD target. Our algorithm is guaranteed to find the optimal solution of the induced DCOPs, which must play an important role in reducing the errors in computing TD target. We also observe that DCG sticks in a bad local optimum with online data collection, but its performance is improved in the offline setting. This result indicates that the hardness of greedy action selection causes DCG to collect low-quality samples in the online setting, which may hurt the final performance. In contrast, our method converges to the same superior value in both settings, highlighting the effectiveness of polynomial-time coordination graphs.

For the second contribution, we show the importance of learning a state-dependent structure. As illustrated in Fig.~\ref{figure:sensor_curves}c, the performance of SOP-CG is much better than both DCG (line) and DCG (star) with online data collection. A static sparse topology usually cannot express the coordination dependencies in all steps, so these methods could not work well even if they are built upon polynomial-time coordination graphs.

\subsection{Performance Comparison}
% \begin{figure}[t]
%     \centering
%     \boxed{TODO}
%     \caption{Illustrations of the three tasks.}
%     \label{figure:env_illustations}
% \end{figure}
\begin{figure}[t]
    \centering
    \vspace{-3mm}
    \includegraphics[width=\linewidth]{figures/performance.pdf}
    \caption{Learning curves on Pursuit, Chasing and Postman. The optimal return is demonstrated if it is available.}
    \label{figure:performance}
\end{figure}

To further demonstrate the effectiveness of our algorithm and discuss the difference among the graph classes, we evaluate SOP-CG on three large-scale complex tasks with highly dynamic coordination requirements and partial observation: Pursuit, Chase and Postman.
\begin{itemize}[leftmargin=25pt]
    \item \emph{Pursuit}. This environment is also called predator-and-prey, which is widely used in recent work \citep{son2019qtran,bohmer2020deep,wang2021context}. 20 agents and 10 random walking prey interact on a $10\times 10$ grid-world. Based on a limited sight range, an agent can move on the map or catch adjacent prey. One prey is captured only if at least two adjacent agents catch it simultaneously, inducing a joint reward of 1. After that, both agents and the captured prey are removed from the game. If only one agent tries to catch the prey, it will fail and receive a punishment of -1.
    \item \emph{Chase}. This is a challenging task on the particle world with trained adversaries instead of built-in AIs created by \cite{lowe2017multi}. On the map with 3 randomly generated obstacles, 10 slower agents chase 3 faster adversaries. For each collision between an agent and an adversary, the agents receive a reward while the adversaries are punished. An agent or adversary can observe the units in a restricted circular area that is centered at its position. We train the agents by a specific algorithm, and the adversaries are concurrently trained by VDN.
    \item \emph{Postman}. $12$ postmen work in a vast community to deliver letters from residents to the post office. With the post office located in the northwest of the community, the whole community is separated into three parts according to the distance to the post office, and each postman will only work in one region. Postmen need to pick randomly generated letters in the community. While two postmen meet each other, any one of them can offer its letters to another one, so they can collaborate in order to deliver the letters to the post office. A postman can observe the information of other postmen and the letters in a sight range.
\end{itemize}

We compare our method with the state-of-the-art coordination graph learning methods (DCG~\citep{bohmer2020deep}, CASEC~\citep{wang2021context}), fully decomposed value-based  methods (VDN~\citep{sunehag2018value}, QMIX~\citep{rashid2020monotonic}) and communication-based method (NDQ~\citep{wang2019learning}). The implementation details and hyperparameter settings are included in Appendix~\ref{appendix:hyperparameter}. As presented in Fig.~\ref{figure:performance}, SOP-CG outperforms the baselines in all three environments.

% On task Pursuit with $20$ agents, our method achieves almost the optimal of this task while DCG has over two times much gap with the optimal value than ours. The reason is that Pursuit needs precise collaborations since if only one agent tries to catch the prey, it will fail and induce a punishment of $-1$. When facing growing scales, DCG has a poor accuracy on DCOP, as we showed before, which may lead to imprecise one-step TD target, impeding DCG to better performance. Notably that, SOP-CG ($\mathcal{G}_P$) has a slightly better performance than SOP-CG ($\mathcal{G}_H$) on this task since Pursuit mainly involves pairwise cooperation, which proves our statement that if the graph class is enough to express the coordination dependency in one task, using such topology will be more efficient. On task chase, our method significantly outperforms fully-decomposed value-based methods and other coordination graph learning algorithms. We can see that value-based algorithms have the poorest performance, and DCG along with CASEC also have similar performance. This declares that the fully connected coordination graph cannot work very well on complex coordination-needed tasks. Furthermore, we can see that SOP-CG($\mathcal{G}_P$) has a better performance than DCG, but much worse than SOP-CG($\mathcal{G}_H$), which can be explained by the lack of representing capacity in SOP-CG($\mathcal{G}_P$). Besides, our method can construct self-organized coordination graphs on this task, you can find the visualization in next subsection. Finally, SOP-CG also works well on a huge comprehensive task.

Using a smaller graph class will be more efficient if such a concise graph class is sufficient to express the coordination dependency in the task of interest. Taking the task Chase as an example, DCG and CASEC performs as poorly as the fully-decomposed methods, as their graph classes are too large and complex to learn. However, our method significantly outperforms coordination graph learning algorithms with a smaller graph class, which strongly confirms our statement. Furthermore, SOP-CG ($\mathcal{G}_T$) has better performance than SOP-CG ($\mathcal{G}_P$) on this task, which may be due to the lack of representational capacity of $\mathcal{G}_P$. On the contrary, Pursuit mainly involves pairwise cooperation, so SOP-CG ($\mathcal{G}_P$) achieves better sample efficiency than SOP-CG ($\mathcal{G}_T$).

We will show that reducing the error of DCOP can also improve performance. On task Pursuit with $20$ agents, our method achieves almost the optimal of this task while DCG has over two times larger gap with the optimal value than ours. The reason is that Pursuit requires precise collaborations. If only one agent tries to catch the prey, it will fail and induce a large punishment. When facing growing scales, DCG and CASEC have a poor accuracy on DCOP, as we showed before, which may lead to inaccurate greedy action selection, impeding DCG to better performance. In the super hard task Postman, which requires agents to collaborate during long horizon, our method also outperforms other methods.

\subsection{Visualization of Self-Organized Coordination}
\begin{figure}[t]
    \centering
    \vspace{-3mm}
    \includegraphics[width=0.9\linewidth]{figures/chase-illustration.pdf}
    \vspace{-0.1in}
    \caption{Various coordination graphs learned by our algorithm on Chase: (a) Self-organized grouping at initialization; (b) Connecting to agent with rich observation for better information sharing; (c) Concentrated collaboration structure around an enclosed adversary.}
    \label{figure:chase_illustration}
\end{figure}

% To illustrate the self-organization property of our method, we take three snapshots chronologically from one episode and build a visualization of the coordination graphs of the three snapshots. As illustrated in Fig.~\ref{figure:chase_illustration}, our method forms various coordination structures in different time-steps, which helps effective collaboration in corresponding situations.  Fig.~\ref{figure:chase_illustration}(a) is the initial of the game; agents and prey spawn randomly on the map. As each agent only focuses on the closest prey, the coordination is separated into three parts according to the nearest prey of each agent. In addition, each agent will connect to the agent in the other direction of the prey if they try to close in the prey, otherwise, it will connect to the agent closest to the prey.  As time goes by, in Fig.~\ref{figure:chase_illustration}(b), two prey throw off the agents and gather at the bottom left of the map since they have a higher speed comparing to the agents. Only agent $1$ can observe the two prey simultaneously, which makes it connect to the majority of the rest of agents and helps the other agents recognize the position of the prey, especially agents $3,4$ and $9$ who lose all prey in their 视野. As illustrated by Fig.~\ref{figure:chase_illustration}(c), finally, one prey is surrounded by multiple agents, which means the agents will receive considerable rewards in a short time. Hence other agents connect to the agents close to the prey and try to keep the surround.

% We visualize the coordination structures learned by SOP-CG ($\mathcal{G}_H$) on Chase to illustrate the self-organization property of our method. As shown in Fig.~\ref{figure:chase_illustration}, we take three snapshots chronologically from one episode. Our method organizes various coordination graphs in different time-steps, which helps effective collaboration in corresponding situations.  Fig.~\ref{figure:chase_illustration}(a) is the initial of the game, where agents and adversaries spawn randomly on the map. As the three adversaries distribute in separate positions, the agents naturally form three groups to chase different adversaries. Notably, both agents $2$ and $7$  collaborate with agent $0$ rather than with each other, as they can try to close in the nearby adversary to make a higher reward. After several time steps, in Fig.~\ref{figure:chase_illustration}(b), two adversaries throw off the agents and gather at the bottom left of the map since they have a higher speed comparing to the agents. Only agent $1$ can observe the two adversaries simultaneously, which makes it connect to the majority of the rest of the agents and helps the other agents recognize the position of the adversaries, especially agents $3,4$ and $9$ who lose all adversaries in their views. As illustrated by Fig.~\ref{figure:chase_illustration}(c), finally, the bottom adversary is surrounded by multiple agents, yielding an opportunity for the agents to win considerable rewards in a short time, which makes the agents form a close collaboration structure around the adversary.

A major strength of our method is that SOP-CG can organize different coordination graphs to adapt to different situations. Such an adaptive organization mechanism can improve the efficiency of multi-agent collaboration. To illustrate the coordination relations organized by SOP-CG, we visualize the learned graph structures on Chase. In Fig.~\ref{figure:chase_illustration}, we take three snapshots chronologically from one episode. This episode is collected by SOP-CG ($\mathcal{G}_T$) using the tree-based graph class. It shows that SOP-CG can produce interpretable graph structures that characterize the ground-truth coordination dependencies. The learned coordination behaviors are interpreted as follows:
\begin{enumerate}[leftmargin=25pt]
    \item Fig.~\ref{figure:chase_illustration}a presents the initial status of the game, where agents and adversaries are generated randomly on the map. As the three adversaries distribute in separate positions, the agents naturally form three groups to chase different adversaries.
    \item After several time steps, in Fig.~\ref{figure:chase_illustration}b, two adversaries gather at the bottom left of the map. Note that, in this game, each agent can only observe objects within a small circular range. Only agent $1$ can observe the two adversaries simultaneously, which makes it connect to the majority of the rest of the agents and helps them recognize the position of the adversaries.
    \item Finally, as illustrated by Fig.~\ref{figure:chase_illustration}c, the bottom adversary is surrounded by multiple agents, yielding an opportunity for the agents to win considerable rewards, which makes the collaboration structure concentrate around the adversary.
\end{enumerate}
% As presented above, the graph structures learned by SOP-CG match the ground-truth demands for effective collaboration on Chase. It demonstrates the ability of our approach to organizing coordination relations.
As presented above, the graph structures learned by SOP-CG can learn effective coordination patterns in Chase, which can be explained by the oracle collaboration strategy of human experts. It demonstrates the ability of our approach to organizing coordination relations.
